DiaTrend: A dataset from advanced diabetes technology to enable development of novel analytic solutions

Objective digital data is scarce yet needed in many domains to enable research that can transform the standard of healthcare. While data from consumer-grade wearables and smartphones is more accessible, there is critical need for similar data from clinical-grade devices used by patients with a diagnosed condition. The prevalence of wearable medical devices in the diabetes domain sets the stage for unique research and development within this field and beyond. However, the scarcity of open-source datasets presents a major barrier to progress. To facilitate broader research on diabetes-relevant problems and accelerate development of robust computational solutions, we provide the DiaTrend dataset. The DiaTrend dataset is composed of intensive longitudinal data from wearable medical devices, including a total of 27,561 days of continuous glucose monitor data and 8,220 days of insulin pump data from 54 patients with diabetes. This dataset is useful for developing novel analytic solutions that can reduce the disease burden for people living with diabetes and increase knowledge on chronic condition management in outpatient settings.

==> datarecords.tex <==
The DiaTrend dataset consists of 54 Excel files--- one file for each subject. Each file has a CGM sheet providing the blood glucose sensing data that was collected by the CGM with 2 columns: date and mg/dl. All the subject files have a Bolus sheet, which describes bolus doses and meal announcements and includes the following 7 columns: date, normal, carbInput, insulinCarbRatio, bgInput, recommended.carb, and recommended.net. Additionally, 37 of those Bolus sheets include 4 more columns: recommended.correction, insulinSensitivityFactor, targetBloodGlucose, and insulinOnBoard. There are 17 subject files that have a Basal sheet describing the subject's basal infusions with the 3 columns: date, duration, and rate. 

Each row in all three of the Excel sheets refers to a sample collected at the timestamp in the column, date. Except for the date column, the rest of the data can be read as floating point numbers.

\begin{table}
% \centering
\begin{tabular}{p{0.05\textwidth} p{0.2\textwidth} | p{0.3 \textwidth} p{0.35\textwidth}}
Sheet Name              & Column Name              & Format                       & Description  \\
\hline \hline
\multirow{2}{*}{CGM}    & date                     & datetime (yyyy-mm-dd HH:MM:SS) & {Date and time that glucose reading was recorded}\\ 
                        & mg/dl                    & Float64                      & Blood glucose reading in mg/dL \\
\hline
\multirow{11}{*}{Bolus} & date                     & datetime (yyyy-mm-dd HH:MM:SS) & Date and time that bolus was administered \\ 
                        & normal                   & Float64                      & Amount of bolus insulin delivered (units) \\ 
                        & carbInput                & Float64                      & Total carbs announced for bolus (grams) \\
                        & insulinCarbRatio         & Float64                      & Patient setting for grams of carbs covered per one unit of insulin \\ 
                        & bgInput                  & Float64                      & Blood glucose reading at time of bolus (mg/dL) \\ 
                        & recommended.carb         & Float64                      & Amount of insulin recommended to cover carb intake for normal bolus \\ 
                        & recommended.net          & Float64                      & Amount of insulin recommended for bolus delivery \\ 
                        & recommended.correction   & Float64                      & Amount of insulin recommended for correction component of normal bolus \\ 
                        & insulinSensitivityFactor & Float64                      & Patient setting for how one unit of insulin lowers blood glucose level \\ 
                        & targetBloodGlucose       & Float64                      & Target blood glucose value for after bolus delivery  \\ 
                        & insulinOnBoard           & Float64                      & Amount of active insulin remaining from prior insulin doses \\
\hline
\multirow{2}{*}{Basal}  & date                    & datetime (yyyy-mm-dd HH:MM:SS) & Date and time of basal infusion\\ 
                        & duration                & Float64                      &  Duration of basal infusion (ms)\\   
                        & rate                    & Float64                      &  Rate of basal infusion (units/hr) 

\end{tabular}
\caption{Description of the sheet names and columns in the dataset.}
\label{Tab:data_records}
\end{table}
